Plasma Physics in Strong Field Regimes

In strong electromagnetic fields, new plasma phenomena and applications emerge, whose modeling requires analytical theories and numerical schemes that I will develop in this thesis. Based on my new results of the classical plasma model, the role of strong magnetic fields during laser-plasma interactions can now be understood. Moreover, based my new quantum electrodynamics (QED) models for plasmas, it is now possible to understand strong-field QED effects in astrophysical environments and test them in laboratory settings.

==> ch-appendicies/printing.tex <==
\chapter{Printing and Binding\label{ch:printing}}

\section{Printing}

For the library copies of your dissertation, you must use archival quality printing and binding. This means acid-free paper, containing at least 25\% cotton fiber. Triangle Repocenter on Nassau Street in Princeton offers both 25\% cotton paper and 100\% cotton paper. Most people choose the 25\% cotton paper, and this is generally recommended by the binders. The 100\% copy paper is somewhat thicker and the extra expense is unnecessary. 

Triangle offers online submission of your printing and binding order at: \url{http://triangleprinceton.com/collegiatebinding/thesis/}. If you request binding from them, they will deliver the paper copies to Smith-Shattuck Bookbinding for you and allow you to pick up the completed copies at their store on Nassau Street. The whole process takes 2-3 business days, but check with them in advance during the busy thesis-printing season in April and May. 

Currently, your printed and bound dissertation copies can be single spaced. Only the electronic copy submitted to ProQuest must be double spaced. All copies must be printed single-sided, with specific margins. 

\section{Binding}

An archival-quality sewn binding is required for the library copies of your dissertation. Smith-Shattuck Bookbinding is highly recommended, and is used by most students. Triangle Repocenter will send your copies there for you, greatly simplifying the process, but you can call Smith-Shattuck with special requests. 

The ``library standard'' sewn binding is sufficient for the copies to be sent to Mudd Library. It uses a black buckram cloth cover, which is the most popular option. For extra copies for yourself and your family members, you can choose ``buckram roundback binding'', which adds decorative lines on the spine, and printing of the title and author on the front cover. For a small additional fee, you can include the Princeton University shield on the front cover and a ribbon bookmark. Leather covers are also available. See Smith-Shattuck's website for more details at: \url{http://www.thesisbookbinding.com/}. 

==> part-3wave/ch-fluid-1st/sec-eigen/wrwc.tex <==
\subsection{Resonances and cutoffs\label{sec:fluid-1st:dispersion:wrwc}}

From previous discussion of wave propagations at special angles, we see a number of special frequencies arise. One set of frequencies are the resonance frequencies, which are the asymptotic values of $\omega$ on electrostatic branches when $ck\rightarrow\infty$. As the frequency approaches the resonance frequencies from the below, the refractive index $n^2\rightarrow\infty$. Divide $n^2$ from $\mathcal{D}'$


so we can find $\omega_r$ by solving $A(\omega_r)=0$. In electron-ion plasma, this equation for resonance frequencies can be explicitly written as
\begin{eqnarray}
	\label{eq:resonance}
	0&=&\omega_r^6-\omega_r^4(\omega_p^2+\Omega_e^2+\Omega_i^2)-\omega_p^2\Omega_e^2\Omega_i^2\cos^2\theta\\
	\nonumber
	&+&\omega_r^2[\omega_p^2(\Omega_e^2+\Omega_i^2)\cos^2\theta-\omega_p^2\Omega_e\Omega_i\sin^2\theta+\Omega_e^2\Omega_i^2].
\end{eqnarray}
The above cubic equation for $\omega_r^2$ has three solutions (Fig.~\ref{fig:Resonance}), which can be ordered from large to small as the upper $(\omega_u)$, lower $(\omega_l)$, and bottom $(\omega_b)$ resonance. When $\theta\sim 0$ or $\pi$, the resonance frequencies approaches $\omega_p, |\Omega_e|$, and $\Omega_i$. Keeping the next order angular dependence, the three resonance frequencies, when $\sin\theta\sim0$, can be approximated by
\begin{eqnarray}
	\label{eq:wu_para}
	\frac{\omega_r^2}{\omega_p^2}&\simeq&1-\frac{\Omega_e^2\sin^2\theta}{\Omega_e^2(2-\cos^2\theta)-\omega_p^2},\\
	\label{eq:wl_para}
	\frac{\omega_r^2}{\Omega_e^2}&\simeq&1-\frac{\omega_p^2\sin^2\theta}{\omega_p^2(2-\cos^2\theta)-\Omega_e^2},\\
	\label{eq:wb_para}
	\frac{\omega_r^2}{\Omega_i^2}&\simeq&1-\frac{\Omega_i}{|\Omega_e|}\tan^2\theta.
\end{eqnarray}
In the other limit, when $\theta\sim \pi/2$, the resonance frequencies approaches the upper-hybrid frequency $\omega_{UH}$, the lower hybrid frequency $\omega_{LH}$, and $0$. Keeping the next order angular dependence, the upper, lower, and bottom resonance frequencies, when $\cos\theta\sim 0$, can be approximated by 
\begin{eqnarray}
	\label{eq:wu_perp}
	\frac{\omega_u^2}{\omega_{UH}^2}&\simeq&1- \frac{\omega_p^2\Omega_e^2\cos^2\theta}{(\omega_p^2+\Omega_e^2)^2+\omega_p^2\Omega_e^2\cos^2\theta},\\
	%\nonumber
	\label{eq:wl_perp}
	\frac{\omega_l^2}{\omega_{LH}^2}&\simeq&1+\frac{\Omega_e^2\cos^2\theta}{\Omega_e^2\cos^2\theta+|\Omega_e|\Omega_i(1+\cos^2\theta)},\\
	%&\simeq&1+\frac{|\Omega_e|}{\Omega_i}\cos^2\theta,\\
	%\nonumber
	\label{eq:wb_perp}
	\frac{\omega_b^2}{\Omega_i^2}%&\simeq&\frac{\omega_p^2\Omega_e^2\Omega_i^2\cos^2\theta}{\Omega_e^2\Omega_i^2-\omega_p^2\Omega_e\Omega_i+\omega_p^2\Omega_e^2\cos^2\theta}\\
	&\simeq&\frac{|\Omega_e|\cos^2\theta}{\Omega_i+|\Omega_e|\cos^2\theta}.
\end{eqnarray}
The above asymptotic expressions for resonance frequency $\omega_r$ are extremely useful when we approximate the scattering strength and wave energy coefficients.



\begin{figure}[t]
	\centering
	\includegraphics[angle=0,width=0.6\textwidth]{part-3wave/ch-fluid-1st/figures/Resonance}
	\caption[Resonance frequencies in magnetizd electron-ion plasma]{Resonance frequencies in electron-ion plasma with $m_i/m_e=10$. In over-dense plasma, eg.~$|\Omega_e|/\omega_p=0.8$ (a), as $\theta$ increases from $0^\circ$ to $90^\circ$, the upper resonance (red) increases from $\omega_p$ to $\omega_{UH}$; the lower resonance (orange) decreases from $|\Omega_e|$ to $\omega_{LH}$; and the bottom resonance (blue) decreases from $\Omega_i$ to zero. In under-dense plasma, eg.~$|\Omega_e|/\omega_p=1.2$ (b), as $\theta$ increases from $0^\circ$ to $90^\circ$, the upper resonance (red) increases from $|\Omega_e|$ to $\omega_{UH}$; the lower resonance (orange) decreases from $\omega_p$ to $\omega_{LH}$; and the bottom resonance (blue) decreases from $\Omega_i$ to zero. This figure can be used to read out the frequency shift $\Delta\omega$, once the scattering angle of the longitudinal wave is known.}
	\label{fig:Resonance}
\end{figure}


==> part-3wave/ch-fluid-1st/sec-model/fluid.tex <==
\subsection{Fluid model as moments of the kinetic equation\label{sec:fluid-1st:model:fluid}}

fluid

==> part-3wave/ch-fluid-1st/sec-model/kinetic.tex <==
\subsection{Kinetic model of classical statistical systems\label{sec:fluid-1st:model:kinetic}}

kinetic model

==> part-3wave/ch-fluid-2nd/sec-general/alternat.tex <==
\subsection{Alternative form of first order equations\label{sec:fluid-2nd:2nd:alternat}}

Alternative


==> part-QED/ch-simulation/sec-latticeQED/Wilson.tex <==
\subsection{Wilson's formulation\label{sec:lattice:Wilson}}

Wilson's line and loop
numerical path integral




==> part-QED/ch-simulation/sec-latticeQED/classical.tex <==
\subsection{The classical statistic regime and real-time simulations\label{sec:lattice:classical}}

classicality condition

real-time simulation

While lattice simulations may be unfamiliar for plasma physics, they have been used extensively in quantum chromodynamics (QCD) to describe the strong interaction \cite{Wilson74} and quark-gluon plasmas \cite{Bass99,Satz00}. In conventional lattice-QCD simulations, quantum correlation functions are computed using numerical path integrals, from which observables are extracted as coefficients of scaling laws \cite{Creutz80}. This scheme can be analytically continued to imaginary time to describe statistical systems in thermal equilibrium \cite{Yagi05}. For out-of-equilibrium systems, real-time simulations can be carried out using the Schwinger-Keldysh time contours \cite{Schwinger61,Keldysh65}. The above formulations, based on numerical path integrals, are capable of capturing genuine quantum loop effects, but are numerically expensive. Fortunately, the computational cost can be dramatically reduced when the occupation numbers of quantum states are high and when the coupling is weak. This is precisely the case for plasma physics, where a large number of particles are present, and the coupling coefficient $e\approx0.3$ is small. In this classical-statistic regime, tree-level effects dominate loop effects \cite{Aarts02,Mueller04,Jeon05,Berges07,Berges14}, and the quantum system can be adequately described by time-advancing the classical field equations with an ensemble of statistically equivalent initial conditions \cite{Aarts99,Gelis13,Polkovnikov03,Borsanyi09}. Based on this approach, lattice spinor-QED simulations have been carried out to demonstrate production of fermion pairs from the vacuum by self-consistent background electric fields \cite{Hebenstreit13,Hebenstreit13String,Kasper14}. However, the role of non-vacuum plasma backgrounds during pair production has not been investigated. %By incorporating a nonperturbative amount of background particle fields, we turn real-time lattice simulations into numerical tools useful for plasma physics. 


In this paper, we demonstrate plasma effects during pair productions using the scalar-QED model. Keeping in mind that the derivation for spinor QED proceeds analogously, the scalar-QED model enables a clean demonstration of collective plasma effects, without the complication of spin and chiral effects associated with Dirac fermions \cite{Nielsen81,Chandrasekharan04,Mueller16a,Mueller16b}. The scalar-QED model governs interactions between electromagnetic (\textit{EM}) fields and spin-0 charged bosons, such as charged pions or Cooper pairs. Although laboratory plasmas are typically made of spin-1/2 charge fermions, classical plasma physics takes no account of particle spin-statistics at all. Therefore, lattice scalar QED, which has been used to study laser-plasma interactions \cite{Eliasson11,Shi16}, provide a sufficient demonstration. In the classical-statistics regime, scalar QED is governed by the Klein-Gordon-Maxwell (KGM) equations
\begin{eqnarray}
	\label{eq:KGMp}
	(D_{\zeta,\mu} D_\zeta^\mu+m_\zeta^2)\phi_\zeta&=&0, \\
	\label{eq:KGMA}
	\partial_\mu F^{\mu\nu}&=&j^{\nu},
\end{eqnarray}
where we have used the natural units $\hbar=c=\epsilon_0=1$. In the above equations, $\phi_\zeta$ is the complex scalar field, describing spin-0 bosons of species $\zeta$, whose charge is $q_\zeta$ and mass is $m_\zeta$. The real-valued 1-form $A_\mu$ is the gauge field, describing spin-1 bosons, and $F_{\mu\nu}=\partial_\mu A_\nu-\partial_\nu A_\mu$ is the field strength tensor. Charged bosons couple to the gauge field through the covariant derivative $D_{\zeta,\mu}=\partial_\mu-iq_\zeta A_\mu$, and the gauge field couples with charged fields through the gauge-invariant current density
\begin{equation}
	\label{eq:j}
	j^\nu=\sum_\zeta\frac{q_\zeta}{i}\big[\bar{\phi}_\zeta(D_\zeta^\nu\phi_\zeta)-\text{c.c.}\big],
\end{equation}
where $\bar{\phi}_\zeta$ denotes complex conjugation of $\phi_\zeta$. By the famous Klein paradox \cite{Klein29}, the charged scalar field $\phi_\zeta$ cannot be interpreted as the probability amplitude of a single particle. A more appropriate interpretation is that the classical field $\phi_\zeta$ is intrinsically a many-particle field, which can be represented as $\phi_\zeta(x)=\int\sqrt{V}\Phi_\zeta(x,x_2,x_3,\dots)$, where $\Phi_\zeta(x,x_2,x_3,\dots)$ is the symmetrized many-body wave function, and the integration is carried out on the many-body configurations space \cite{Shi16}. Regardless of the interpretation, we can solve the KGM equations as coupled partial differential equations, whose solutions model the tree-level behavior of charged bosons interacting with \textit{EM} fields.  



==> part-QED/ch-simulation/sec-latticeQED/statistics.tex <==
\subsection{Statistical systems in thermal equilibrium\label{sec:lattice:statistics}}

Wick rotation imaginary time
thermal ensemble


